Technical Report: Time-Bounded Resilience

Most research on formal system design has focused on optimizing various measures of efficiency. However, insufficient attention has been given to the design of systems optimizing resilience, the ability of systems to adapt to unexpected changes or adversarial disruptions. In our prior work, we formalized the intuitive notion of resilience as a property of cyber-physical systems by using a multiset rewriting language with explicit time. In the present paper, we study the computational complexity of a formalization of time-bounded resilience problems for the class of $\eta$-simple progressing planning scenarios, where, intuitively, it is simple to check that a system configuration is critical, and only a finite number of actions can be carried out in a bounded time period. We show that, in the time-bounded model with $n$ (potentially adversarially chosen) updates, the corresponding time-bounded resilience problem for this class of systems is complete for the $\Sigma^P_{2n+1}$ class of the polynomial hierarchy, PH. To support the formal models and complexity results, we perform automated experiments for time-bounded verification using the rewriting logic tool Maude.

==> report-only/delta-representations-PTS.tex <==
%\vspace{-2mm}
%In this section we investigate the complexity of the verification problems  defined in Section~\ref{sec:bounded} for progressing timed systems.
%
%In order to obtain the complexity results for the corresponding verification problems, we use the machinery introduced in our previous work~\cite{kanovich.mscs} called $\delta$-representations.

\vspace{5pt}
\subsection{$\delta$-representations}\label{sec:delta}


Some of our results, for a given planning scenario $A=(\Rscr,\GS,\CS,\Escr,\Sscr_0)$, we will mention the value $\Dmax$ which is an upper-bound on the natural numbers appearing in $\Sscr_0, \Rscr, \Escr,\GS$ and $\CS$. The value of $\Dmax$ can be inferred syntactically by simply inspecting the timestamps of $\Sscr_0$, the $D$ values in timestamps of rules (which are of the form \ $T + D$) and constraints in $\CS$, $GS$ and in rules of $\Rscr$ and $\Escr$ (which are of the form $T_1 > T_2 \pm D$, $T_1 = T_2 \pm D$ and\, $T_1 \geq T_2 \pm D$). 
%For example, the $\Dmax = 1$ for the specification in Figure~\ref{fig:rules-complete}.

For our  results we  assume a bound on the size of facts.
%For example, in our specification in Figure~\ref{fig:rules-complete}, we can take the bound ~$k= |x_{max}| +|y_{max}|+ |e_{max}|+5$.
%
Notice, however, that we do not always impose an upper bound on the values of timestamps. 
%Also, we allow an unbounded number of fresh values to appear in a trace. 




\begin{definition}
\label{def: delta-representation}
Let  \, $ \Sscr = \{\,Q_1@t_1, \,Q_2@t_2, \ldots, \,Q_n@t_n \,\} $
be a configuration of a timed MSR $\Tscr$
written in canonical way where the sequence of
timestamps $t_1, \ldots, t_n$ is non-decreasing. 
(For the case of equal timestamps, we sort the facts in alphabetical order, if necessary, except that we put $\Time$ first.) 
The \emph{$\delta$-representation} of $\Sscr$ for a given $\Dmax$ is 
$$
\delta_{\Sscr,\Dmax} = [~Q_1,\,\delta_{Q_1,Q_2},\,Q_2, \ldots, \,Q_{n-1}, \,\delta_{Q_{n-1},Q_n}, \,Q_n~] \ .
$$
Here, for a given natural number $\Dmax$, \ $\delta_{P,Q}$ \ is the \emph{truncated time difference} of two timed facts
~$P@t_1$ and $Q@t_2$~ with \mbox{$t_1\leq t_2$}, defined as follows:
$$
\delta_{P,Q} = 
\left\{\begin{array}{ccl}
t_2 - t_1 & , & \ \textrm{ provided } ~t_2 - t_1 \leq \Dmax\\
\infty & , & \ \textrm{ otherwise } 
\end{array}\right. \ .
$$
\end{definition}

%\vspace{0,5em} \noindent
For simplicity, when $\Dmax$ is clear from the context, we sometimes write $ \delta_{\Sscr}$ instead of ~$ \delta_{\Sscr,\Dmax}$.

\vspace{0,5em}
In our previous work~\cite{kanovich12rta,kanovich.mscs}, we showed that a $\delta$-representation is an equivalence class on configurations. Namely, for a given $\Dmax$, we declare $\Sscr_1 $ and $ \Sscr_2$ equivalent, written ~$\Sscr_1 \equiv_{\Dmax} \Sscr_2$, 
if and only if their $\delta$-representations are exactly the same.
%(\st{up to nonce renaming}, \ie, \st{~$\Sscr_1 \sigma = \Sscr_2$, where $\sigma$ is a bijection on the set of nonce names}).



\vspace{0,5em}
This equivalence relation is well-defined with respect to time constrains, \ie, ~configurations that have the same $\delta$-representation satisfy exactly the same set of constraints.
Here, when saying that configurations satisfy the same constraint, we implicitly mean that time variables of the constraint refer to the same facts in both configurations.
Therefore, we can say that a $\delta$-representation satisfies a constraint or does not. Similarly, we say that a $\delta$-representation is critical iff it is the $\delta$-representation of a critical configuration and that  a $\delta$-representation is a goal $\delta$-representation iff it is the $\delta$-representation of a goal configuration.


Also, the equivalence among configurations is well-defined with respect to application of rules, \ie, ~application of rules on $\delta$-representations is unambiguous. Therefore we can consider traces over $\delta$-representations. 
For details on the concrete procedure of how to apply a rule on a given $\delta$-representation see~\cite[Section 4.3]{kanovich.mscs}.
%
{\color{blue}
%Recall that 
Rules over abstractions model rules over corresponding concrete configurations. Technically, they transform $\delta$-representations, by changing the facts and the truncated time distances in a sequence

$
%\delta_{\Sscr,\Dmax} =
[~Q_1,\,\delta_{Q_1,Q_2},\,Q_2, \ldots, \,Q_{n-1}, \,\delta_{Q_{n-1},Q_n}, \,Q_n~] \ .
$
\\
In particular, the $Tock$ rule over $\delta$-representations  corresponding to the $Tick$ 
% The time  $Tock$ rule is similarly applied for other cases, see
is shown in Figure~\ref{fig:Tock}.
}
\begin{figure}[t]
    %\centering
    $
    \begin{array}{lrc}
      \lbrack~F_1=\Time, 0, F_2,  \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n},
0, F_i,0, \ldots
\,0, F_n~\rbrack
\lra  
%\\ \qquad
      \lbrack~F_2, 0, \dots,0, F_{n},1,\Time~\rbrack
\\[5pt]
     \lbrack~F_1=\Time, %0, F_2,
     \ldots 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n},
, F_i, \delta_{F_{i},F_{i+1}}, F_{i}, \ldots
\,F_n~\rbrack
\lra  
\\ \qquad
      \lbrack~F_2, 0, \dots,0, F_{i-1},1,\Time, \delta_{F_{i},F_{i+1}}-1, F_{i+1} \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
\,F_n~\rbrack\\ 
\hfill \text{if } \ ~\delta_{F_{i},F_{i+1}}>0, ~ ~\delta_{F_{1},F_{2}}0=\delta_{F_{i-1},F_{i}}=0
\\[5pt]
    \lbrack~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, F_{i-1}, \delta_{F_{i-1},F_i}, F_i=\Time, \delta_{F_{i},F_{i+1}}, F_{i+1} \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
\,F_n~\rbrack
\lra  
\\ \qquad
      \lbrack~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, F_{i-1}, \delta_{F_{i-1},F_i}+1, F_i=\Time, \delta_{F_{i},F_{i+1}}-1, F_{i+1} \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
\,F_n~\rbrack\\ 
\hfill \text{if } \ ~\delta_{F_{i-1},F_i}< \Dmax, ~\delta_{F_{i},F_{i+1}}>0
\\[5pt]
 \lbrack~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, F_{i-1}, \infty, %\delta_{F_{i-1},F_i}
  F_i=\Time, \delta_{F_{i},F_{i+1}}, F_{i+1} \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
\,F_n~\rbrack
\lra  
\\ \qquad
      \lbrack~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, F_{i-1}, %\delta_{F_{i-1},F_i}+1
      \infty, F_i=\Time, \delta_{F_{i},F_{i+1}}-1, F_{i+1} \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
\,F_n~\rbrack\\ 
\hfill \text{if } \ %~\delta_{F_{i-1},F_i}= \Dmax,
~\delta_{F_{i},F_{i+1}}>0
\\[5pt]
 \lbrack~F_1, %\,\delta_{F_1,F_2},\,F_2,
 \ldots, F_{i-1}, \infty, %\delta_{F_{i-1},F_i}
  F_i=\Time, 0, \ldots , \delta_{F_{i},F_{i+1}}, F_{i+1} \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
\,F_n~\rbrack
\lra  
\\ \qquad
      \lbrack~F_1, %\,\delta_{F_1,F_2},\,F_2, 
      \ldots, F_{i-1}, %\delta_{F_{i-1},F_i}+1
      \infty, F_{i+1}, \dots,0, F_{i+j}, 1, \Time,   \delta_{F_{i+j},F_{i+j+1}}-1, F_{i+j+1}, \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
\,F_n~\rbrack\\ 
\hfill \text{if } \ %~\delta_{F_{i-1},F_i}= \Dmax,
~\delta_{F_{i+j},F_{i+j+1}}>0, ~\delta_{F_{i},F_{i+1}}0=\delta_{F_{i+j-1},F_{i+j}}=0
\\[5pt]
 \lbrack~F_1, %0, F_2,
     \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n},
 \delta_{F_{n-1},F_{n}},
\,F_n=\Time~\rbrack
\lra  
%\\ \qquad
      \lbrack~F_1, \dots,F_{n-1}, \delta_{F_{n-1},F_{n}}+1,\Time~\rbrack\\ 
\hfill \text{if } \ ~\delta_{F_{n-1},F_{n}}<\Dmax
%, ~ ~\delta_{F_{1},F_{2}}0=\delta_{F_{i-1},F_{i}}=0
\\[5pt]
 \lbrack~F_1, %0, F_2,
     \ldots, 
%\,F_{n-1}, \,\delta_{F_{n-1},F_n},
 F_{n-1},\infty,
\,F_n=\Time~\rbrack
\lra  
%\\ \qquad
      \lbrack~F_1, \dots,F_{n-1},\infty,\Time~\rbrack
    \end{array}
    $
        %\includegraphics[width=0.9\textwidth]{resili.pdf}
    \caption{Illustration of time advancement over abstarctions: $Tock$ rules over $\delta$-representations.}
    \label{fig:Tock}
\end{figure}

%\vspace{0.5em}
We naturally extend the notion of a compliant trace and say that a trace over \mbox{$\delta$-representations} is compliant iff it does not contain any critical $\delta$-representation.
%Also, we say that a trace over $\delta$-representations uses the \lts %lazy time sampling 
%if $Tick$ rule is applied to a $\delta$-representation in that trace only when no instantaneous rule is applicable.



Moreover, in~\cite[Theorem 4.1]{kanovich.mscs} we have shown that there is a bisimulation between (compliant) traces over configurations and (compliant) traces over their $\delta$-representations in the following sense:
\
%\hspace{-1em}
~$\Sscr_1 \lra_* \Sscr_2$ \ \ iff \ \ $  \delta_{\Sscr_1} \lra_*   \delta_{\Sscr_2}$ .




%\vspace{0.5em}
When  considering concrete problems and corresponding bisimulations, the bound $\Dmax$ is inferred from numerical values appearing in the problem specification.
This ensures that all configurations in traces are \emph{future bounded}, \ie, do not contain facts $F@t_F$ such that $\delta_{Time,F}= \infty$. This is important for faithful representation of time advances.
{\color{blue}For this reason, the $Tock$ rules in Figure~\ref{def:progressing-delta} are given only for $\delta$-representations that correspond to future bouded configurations. For more details see~\cite[Section 4.3]{kanovich.mscs}.
}

%For self-containment of the paper, in the proof of the following result from~\cite{kanovich16formats} we present main proof ideas used in~\cite{kanovich.mscs} and, moreover, we additionally address the \lts
%lazy time sampling.

The following bisimulation result directly follows from the result obtained in ~\cite{kanovich2021Guttman}.

\begin{proposition}
\label{thm:delta configurations}\cite{kanovich2021Guttman}
For any planning scenario $A=(\Rscr,\GS,\CS,\Escr,\Sscr_0)$ the equivalence relation between configurations is well-defined with respect to the rules of $\Rscr$ and $\Escr$
%of the system (including time advances), 
%the \lts %lazy time sampling 
and goal and critical configurations. 
\\
Namely, to any compliant trace starting from the given initial configuration $\Sscr_0$ 
corresponds a compliant trace over $\delta$-representations starting from $\delta_{\Sscr_0}$. 
%In particular, a trace over configurations uses the \lts
%%lazy time sampling 
%iff the corresponding trace over $\delta$-representations uses the \lts
%%lazy time sampling.
%%~\cite{kanovich16formats}
\end{proposition}

{\color{blue}
When considering planning scenarios with only progressing rules, we ensure the
correctness and completeness of the bisimulation w.r.t. the progressing condition, \ie, we show that the corresponding trace over abstractions is progressing as well.



%For example, the $Tock$ rule over $\delta$-representations  corresponding to the $Tick$ rule transforms 
%
%~$[~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, F_{i-1}, \delta_{F_{i-1},F_i}, F_i=Time, \delta_{F_{i},F_{i+1}}, F_{i+1} \ldots, 
%%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
%\,F_n~] $, 
%\\
%where ~$\delta_{F_{i-1},F_i}< \Dmax$~ and ~$\delta_{F_{i},F_{i+1}}>0$, ~into 
%
%~$[~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, F_{i-1}, \delta_{F_{i-1},F_i}+1, F_i=Time, \delta_{F_{i},F_{i+1}}-1, F_{i+1} \ldots, 
%%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
%\,F_n~] $~.
%\\
%Similarly, the $Tock$ rule   transforms 
%
%~$[~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, F_{i-1}, \Dmax, F_i=Time, \delta_{F_{i},F_{i+1}}, F_{i+1} \ldots, 
%%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
%\,F_n~] $, 
%\\
%where ~$\delta_{F_{i},F_{i+1}}>0$, ~into 
%
%~$[~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, F_{i-1}, \infty, F_i=Time, \delta_{F_{i},F_{i+1}}-1, F_{i+1} \ldots, 
%%\,F_{n-1}, \,\delta_{F_{n-1},F_n}, 
%\,F_n~] $~.




\vspace{5pt}
We now define progressing traces over abstractions that will represent concrete traces which are progressing. Recall that progressing rules over configurations are balanced, cannot consume future facts and create at least one future fact (Definition~\ref{def:progressing}).

\begin{definition}[Progressing Traces over $\delta$-representations]
\label{def:progressing-delta} \ \\
A rule $r$ over $\delta$-representations is \emph{progressing}~ if the following holds:
%for all instantaneous rules $r \in \Tscr$:
\begin{itemize}
\item[i)] Rule $r$ transforms $\delta$-representation $\Delta_1 = [~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, \,F_{n-1}, \,\delta_{F_{n-1},F_n}, \,F_n~] $ into $\delta$-representation
$\Delta_2 = [~Q_1,\,\delta_{Q_1,Q_2},\,Q_2,  \ldots, % Q_j=Time, \ldots,
\,Q_{n-1}, \,\delta_{Q_{n-1},Q_n}, \,Q_n~] $;

\item[ii)] Rule $r$ does not consume any future facts:\\
If $F_i=\Time$ in $\Delta_1$ and $Q_j = \Time$ in $\Delta_2$, then
there is an injective mapping  $f:\{F_{i+1}, \dots, F_n\} \to \{Q_{j+1}, \dots, Q_n\}$ such that 
%for each $F_k, i \in \{i+1, \dots, n\}$ there is $F'_k= Q_l$ in $\Delta_2$~ such that % $j>s$, where $Q_s = Time$, and  \
$\delta_{F_{i},F_{k}} = \delta_{F_{j},f'(F_{k})}$, ~for all $ k \geq i$;
%$\delta_{F_{k},F_{l}} = \delta_{F'_{k},F'_{l}}$, ~for all $ k,l\geq t$;

\item[iii)] Rule $r$ creates a future fact:\\
If $F_i=\Time$ in $\Delta_1$ and $Q_j=\Time$ in $\Delta_2$, then $j<i$
%there is least one ~$Q_i, i \in \{t+1, \dots, n \}$ %in $\Delta_2$ 
%such that $\delta_{Q_{j},Q_i} >0$;
and
$$\displaystyle \sum_{k=i}^{n-1}\delta_{F_{k},F_{k+1}} < \sum_{k=j}^{n-1}\delta_{Q_{k},Q_{k+1}} 
\ \ ( \ \text{ or equivalently } \ \sum_{k=i}^{n-1}\delta_{F_{i},F_{k+1}} < \sum_{k=j}^{n-1}\delta_{Q_{j},Q_{k+1}} ).$$

%Rule $r$ consumes \emph{only} facts with timestamps in the past or at the current time, \ie, in (Eq.~\ref{eq:instantaneous}), the set of constraints ~$\Cscr$ contains the set  $$\Cscr_r = \{~T \geq T_i' \mid F_i@T_i', ~1 \leq i \leq n~\} \ . $$
\end{itemize} 
A trace $\tau$ over $\delta$-representations is \emph{progressing} if all the rules in $\tau$ are %either 
progressing. % or  $Tock$ rules.
\end{definition}

Note that the first condition denotes the balancing property. The second condition ensures that all future facts in the enabling abstraction are not affected by the rule, \ie, they are present in  the resulting abstraction, with the same truncated time difference to the global time. The third condition denotes that at least one future fact is created. Note that the choice of $\Dmax$ numerical bound ensures that the configurations in the traces we consider are not future bounded. Hence, above sums are finite.

\begin{remark}
Note  that the $Tock$ rules %could be considered 
are progressing. % as a borderline case of Definiton~\ref{def:progressing-delta}.
\end{remark}


\begin{remark}
It can be shown that one can check in polynomial time in the size of the planning problem whether a rule over $\delta$-representations is progressing.
\end{remark}


\begin{proposition}[Bisimulation of PTSes]
\label{thm:delta-progressing}\ \\
For any planning scenario $A=(\Rscr,\GS,\CS,\Escr,\Sscr_0)$ the equivalence relation between configurations is well-defined with respect to progressing condition.
\\
Namely, to any compliant trace of the progressing rules of $\Rscr$ and $\Escr$  from the given initial configuration $\Sscr_0$ to a goal configuration $\Sscr_G$
corresponds a compliant progressing trace over $\delta$-representations  from $\delta_{\Sscr_0}$ to $\delta_{\Sscr_G}$. 
\end{proposition}
\begin{proof}
Let $\Dmax$ be a numeric upper-bound on the natural numbers appearing in $\Sscr_0, \Rscr, \Escr,\GS$ and $\CS$.
Assume
%$\Sscr_1$ and $\Sscr_2$ are equivalent configurations, and assume 
that configuration $\Sscr_1$ is transformed to $\Sscr_2$ by means of
a progressing rule~$\alpha$.
Then, according to the bisimulation result %from
\mbox{\cite{kanovich17mscs}[Theorem 4.1]}, there exists a rule $r_{\alpha}$ over  $\delta$-representations that transforms 
$\Delta_1 = \delta_{S_1, \Dmax}$  to 
$ \Delta_2 = \delta_{S_2, \Dmax}$,
as shown in the diagram below:
%Recall that equivalent configurations satisfy the same set of constraints.
%Hence, the rule~$\alpha$ is applicable to $\Sscr_2$ and will transform  $\Sscr_2$ into some $\Sscr_2'$:
\[
\begin{array}{cccc}
\Sscr_1 & \to_{\alpha}& \Sscr_2\\[4pt]
%\biginterleave \
 \wr \ 
& &  \wr\\[4pt]
\Delta_1 &  ~\to_{r_{\alpha}}  & \ \Delta_2
\end{array}
\]
We now show that $r_{\alpha}$ is progressing. % rule over  $\delta$-representations.

For the case when $\alpha$ a $Tick$ rule, the corresponding rule $r_{\alpha}$ an instance of the $Tock $ rule which is shown to be progressing by case inspection of the rules in Figure\ref{fig:Tock}.

%If $\alpha$ is a $Tick$ rule, the corresponding $r_{\alpha}$ rules is the $Tock $ rule, which is a progressing rule according to Definition~\ref{def:progressing-delta}.
When  $\alpha$ is an instantaneous balanced rule, configurations $\Sscr_1$ and $\Sscr_2$ have the same number of facts, hence $\Delta_1=[~F_1,\,\delta_{F_1,F_2},\,F_2, \ldots, \,F_{n-1}, \,\delta_{F_{n-1},F_n}, \,F_n~]$ and 
\mbox{$\Delta_2= [~G_1,\,\delta_{G_1,G_2},\,G_2, \ldots, \,G_{n-1}, \,\delta_{G_{n-1},G_n}, \,G_n~]$} have the same number of facts. Hence, the first condition of Definition~\ref{def:progressing-delta} is satisfied.
The second condition of  Definition~\ref{def:progressing-delta} is also satisfied because $\alpha$ is progressing, so no future facts from $\Sscr_1$ nor the fact $\Time@t$ are consumed by $\alpha$. That is, if $\Time@t, F_i@t_i \in \Sscr_1$ for $t_i >t$, then $\Time@t, F_i@t_i \in  \Sscr_2$, so the condition on the equal time differences between the corresponding future facts of $\Delta_1 $ and $\Delta_2$ holds since it holds for the same future facts in  $\Sscr_1$ and $\Sscr_2$.

For the third condition of Definition~\ref{def:progressing-delta} $j<i$ holds because of the form of instantaneous rules, (\ref{eq:instantaneous-balanced}) and since no future facts are consumed.
Namely,  both configurations have exactly $n$ facts, and only facts in the present and future are created.
Furthermore, sice $\alpha$ created at least one future fact, at least one of the facts $F_l, l<i$ does not appear in $\Delta_2$, hence at least one fact is created and appears as $Q_k, k>j$, with ~$\delta_{Q_j, Q_k}>0$.

%We consider the two types of rules for $\alpha$, namely,  time advances and instantaneous rules.


%Since equivalent configurations satisfy the same set of constraints, 
%$\Sscr_1$ is a goal (critical) configuration if and only if $\Sscr_2$ is a goal (critical) configuration, \ie,~ if and only if $\delta_{\Sscr_1}$ is a goal (critical)  $\delta$-representation. 

Conversely, if $r$ is a progressing rule over  $\delta$-representations that transforms $\Delta_1 $ to$ \Delta_2$, then, as per \mbox{\cite{kanovich17mscs}[Theorem 4.1]}, there exists corresponding configuarations $\Sscr_1$ and $ \Sscr_2$ such that $\Delta_1 = \delta_{S_1, \Dmax}$  and
$ \Delta_2 = \delta_{S_2, \Dmax}$,
and a rule $\alpha$ that transforms $\Sscr_1$ to $ \Sscr_2$.
Since $r$ is progressing, $\Delta_1 $ and $ \Delta_2$ contain the same number of facts, $n$. Then, $\Sscr_1$ and $ \Sscr_2$ also contain $n$ facts,  consequently, $\alpha$ is a balanced rule.

Since $r$ satisfies the second condition of  Definition~\ref{def:progressing-delta}, all future facts from $\Delta_1$, \ie, from $\Sscr_1$ are not consumed.

Finally, as $r$ satisfies the third condition of  Definition~\ref{def:progressing-delta}, % in particular $j<i$,
it follows that $r$ has created at least one fact with timestamp greater than the global time. Therefore, the corresponding rule $\alpha$ creates at least one future fact.


By induction on the length of the (sub)trace, it  follows that, given a progressing planning scenario, 
any %(possibly infinite) 
trace over concrete configurations is compliant and reaches a goal configurations if and only if the corresponding trace over $\delta$-representations is compliant and reaches a goal  $\delta$-representation.
\qed \end{proof}
}


==> report-only/travel-resilience.tex <==

\omitthis{

ab is implicit in the end of the latest event
b being the duration of the last event,
since at that point no more actions can take place.


put discussion of nab alg at the beginning

time sampling diff 

delta is true

We thank Vivek Nigam for many insightful 
discussions during the early part of this work.

#Compare to time bounded recoverability

clarify a is the end of the last event

make clear forall exist representations

}

\section{Travel System Resilience Experiments}
\label{sec:travel-resilience}

To experiment with resilience in practice we
specified the travel system in the Maude rewriting
logic language \cite{maude-book}. In contrast to
the multiset rewriting representation, the Maude
specification uses data structures rather than
facts to represent system structure and state. Also
passing of time is modeled essentially by rule
duration.  For example, rule that models taking a
flight takes time according the duration of the
flight.  Effectively, these rules combine a instantaneous
rule with a time passing rule.
These design decisions together with
relegating as much as possible to equational
reasoning help to reduce the search state space.

We implemented an algorithm to check nab-resilience
for travel system scenarios in which the goal is
to attend a given set of events.  System updates 
change flight schedules and goal updates change event
start or duration or may add an event.
Execution traces terminate when the last event is attended
or an event is missed.  Thus for simplicity we fix
a+b to be  the end of the last possible event and leave
it implicit. 



In the following we describe the representation
of key elements of the travel system specification:
system state, execution rules and the updates.  We then 
explain the algorithm for checking nab-resilience and
report on some simple experiiments.

\subsection{Representing travel status}

There are two main sorts in the travel system specification:
\texttt{Flight} and \texttt{Event}. A flight is
represented by a term
\texttt{fl(cityD,cityA,fn,depT,dur)}. Here
\texttt{cityD} and \texttt{cityA} are the departure
and arrival cities, \texttt{fn} is the flight
number (a unique identifier),
\texttt{depT} is the departure time, and
\texttt{dur} is the duration. The departure time and
duration are represented by hour-minute terms
\texttt{hm(h,m)}. For simplicity, flights are
assumed to go at the same time every day, and all
times are GMT to avoid dealing with time zones.

A flight instance (sort \texttt{FltInst})
represents a flight on a specific date by a term:
\texttt{fi(flt,dtDep,dtArr)} where \texttt{flt} is a
flight, \texttt{dtDep} and \texttt{dtArr} are
date-time terms representing the date and time of
departure and arrival respecively. A date-time term
has the form \texttt{dt(yd,hm)} where \texttt{yd} is
a year-day term \texttt{yd(y,d)} and \texttt{hm} is
an hour-minute term as above.

An event is represented by a term
\texttt{ev(eid,city,loc,yd,hm,dur,opt)}
where \texttt{eid} is a unique identifier (a string), \texttt{opt} is a boolean specifying
whether the event is optional. The other arguments
are as above.

\longversion{
We form lists of flights (sort \texttt{FlightL}),
sets of flight lists (sort \texttt{FltLS}), flight
instance lists (sort \texttt{FltInstL}), sets of
flight instance lists (sort \texttt{FltLS}) and
sets of events (sort \texttt{Events}) as usual
using associative, commutative and id axioms.
}

A system execution state is represented by
a term  of the form
 \verb|{conf}| (sort \texttt{Sys}) where \texttt{conf}
 (sort \texttt{Conf})
is a multiset of configuration elements.
There are three sorts of configuation element:
\texttt{TConf}, \texttt{Log}, and  update desctriptions.
\longversion
{A system state is required to have
one \texttt{TConf} element, and there can be
at most one log and one update element.}

Terms of sort \texttt{TConf} represent a single traveler's state.   They have one of three forms
\begin{small}
  \begin{verbatim}
      tc(dt,city,loc,evs)   --- planning
      tc(dt,city,loc,evs,ev,fltil) --- executing
      tcCrit(dt,city,loc,evs,ev,reason) --- critical
  \end{verbatim}
\end{small}

\noindent
Here \texttt{dt} is a date-time term, the travelers
current date and time, and \texttt{city} tells
what city the traveler is currently in. The term
\texttt{loc} gives the location within the
city, either the \texttt{airport} or the city
\texttt{center}.  \texttt{evs} is
the set of events to be attended while \texttt{ev} is the next event to consider
and \texttt{fltil} is the flight instance list
chosen to get from \texttt{city} to the location
of \texttt{ev}.  The constructor \texttt{tcCrit}
signals a critical configuration, a required event has been missed.  

An update description is a term of the form
\texttt{di(digs)} or \texttt{di(digs,n)} where \texttt{digs}
is a set of digressions. Each digression describes an update
to be applied by an update rule, and \texttt{n} bounds the
number of updates that can be applied.

Two kinds of updates are currently implemented:
flight/system updates and event/goal updates.
The flight updates are
\begin{itemize}
\item
 \texttt{cancel} --- cancel the current flight 
\item
  \texttt{delay(hm(h,m))}  --- delay the current flight by \texttt{hm(h,m)}
\item
   \texttt{divert(city0,city1)} --- divert the current flight to \texttt{city1} (scheduled to arrive  at \texttt{city0}) .
\end{itemize}
  
\noindent
where the current flight is the first
element of the flight instance list of an
executing \texttt{TConf} term.

The event/goal updates  are
\begin{itemize}
\item
  \texttt{edEvS(hm(h,m)} --- start the current event h hours, m minutes earlier
\item
 \texttt{edEvD(hm(h,m))} --- extend the current event duration by h hours, m minutes 
\item
  \texttt{addEv(eid)} --- add the event identified by \texttt{evid} to the set of pending events.
\end{itemize}

\noindent
Since we are concerned with system resilience, not properties
of the traveler, the traveler simply goes to the airport
and looks for available flights to get to the next
event. Flight updates are only applied to the next
flight the traveler is about to take.  Similarly,
the changes in event start time or duration are only
applied to the next event to attend. Many more
complex variations are possible.

An element of sort \texttt{Log} is a list of log items. It
is used to record updates, flights taken, and events
attended or missed. Among other things, when searching for
flights, it is used to know which flights have been
cancelled.

\subsection{Rewrite rules}
There are 5 rules for normal execution 
(\texttt{plan}, \texttt{noUFlts},\texttt{flt}, \texttt{event},
\texttt{replan}) and two
update rules, \texttt{fltDigress} for flight/system updates and \texttt{evDigress} for event/goal updates.

The \texttt{plan} rule, picks
the event, \texttt{ev}, with the earliest start time  from \texttt{nevs} and
(non-deterministically) selects a list of flight
instances, \texttt{fltil}, from the set of all
flight instance lists that arrive at the city of
\texttt{ev} before the event start time. The set of
possible flights is stored in a constant
\texttt{FltDB}. \texttt{log1} is \texttt{log} with
 an item recording the rule firing added.
The conditional \texttt{if ...} does all the computing
mentioned above.
\begin{small}
\begin{verbatim}  
 crl [plan]:
  tc(dt,city, loc, nevs) log
  =>
  tc(dt, city, loc, evs0, ev, fltil) log1
  if ...
\end{verbatim}  
\end{small}
The rule \texttt{noUFlts} takes care of the case
that there is no usable flight instance list
given the current traveler time and location and the time and location of the next event.  
If \texttt{ev} is
optional then it is simply dropped (recording this
in the log) and the rule \texttt{plan} can be
applied to the remaining events.  If \texttt{ev} is
required, then the configuration becomes critical, and
execution terminates.
\omitthis{
\begin{small}
\begin{verbatim}  
 crl[noUFlts]:
  tc(dt,city, at, nevs) log
  =>
  (if getOpt(ev)
  then tc(dt,city,at,evs0) log ; li(getId(ev),false)
  else tcCrit(dt, city, at, evs0, ev, NoUsableFltl") log
  fi)
  if {evs0,ev} := nextEv(nevs)
\end{verbatim}  
\end{small}
}
The rule \texttt{flt} models taking the next flight,
assuming the flight departure time is later than the
traveler's current time.  The traveler's time is
updated to the flight arrival time \texttt{dtArr},
city is updated to the destination \texttt{city1},
and the flight instance taken is removed from the list.
Again, the conditional \texttt{if ...} does all the 
necessary computing.
\begin{small}
\begin{verbatim}  
crl [flt]:
  {tc(dt, city0, airport, evs,ev,flti ; fltil) conf}
  =>
  {tc(dtArr, city1, airport, evs,ev, fltil) conf1
  if  ....
\end{verbatim}  
\end{small}

\noindent
The \texttt{event} rule (not shown) models
attending the currently selected event. It can be
applied when the
traveler city is the same as the event city and the
current time is not after the event start. As for
the flight rule, the current time is updated to the
event end time and the traveler returns to the
airport.  If the traveler arrives at the event
city too late, as for the \texttt{noUFlts} rule,
if the event is optional, the \texttt{event} rule drops the event and enters a log item, otherwise
it produces a critical \texttt{TConf}.

\omitthis{
\begin{small}
\begin{verbatim}  
**** attend the event if in time
 crl [event]:
  {tc(dt, city0, airport, evs,ev,fltil) conf}
  =>
  {conf1}
\end{verbatim}  
\end{small}
}
The \texttt{replan} rule takes care of the situation
when the traveler city is not the event city  
and the next flight, if any, does not deparat from the traveler city or has been missed.  The pending flight
instance list is dropped, the event is put back in
the event set, and a log item
is  added to the log.

\omitthis{
\begin{small}
\begin{verbatim}  
 crl [replan]:
  {tc(dt, city0, airport, evs,ev,fltil) conf}
  =>
  {tc(dt, city0, airport, evs ev) conf1 }
  if ...   .
\end{verbatim}  
\end{small}
}


The update rule \texttt{fltDigress} only applies if
the digression counter is greater than zero and the
rule decrements the counter.  A flight digression,
\texttt{fdig}, is non-deterministically selected from
the available digressions (the first argument to \texttt{di}). 

\begin{small}
\begin{verbatim}  
 crl [fltDigress]:
   { tconf di(fdig digs, s n)  conf}
   =>
   { tconf1 di(digs fdig,n) conf1 }
  if tc(dt, city0, airport, evs,ev, flti ; fltil) := tconf
  /\ city0 =/= getCity(ev)
  /\ tconf1 conf1 := applyDigression(tconf,conf,fdig)
 [print "\nflight digression  " flti "\n fdig " fdig] 
 .   
\end{verbatim}  
\end{small}

\noindent
The first condition exposes the structure of 
\texttt{tconf} to ensure there is a pending
flight to update.  
The auxiliary function \texttt{applyDigression}
specifies the result of the update.  For example
the \texttt{cancel} update removes \texttt{flti} from
the list and adds a log item recording that this
flight instance is cancelled.   
The case where the update description has the
form \texttt{di(fdig digs)} is similar, except
here \texttt{fdig} is removed when applied,
and updating stops when there are no more update
elements in the set.

Similarly the  rule \texttt{evDigress} non-deterministically
selects an event digression from the configuration's
digression set and uses the auxiliary function
\texttt{applyEvDigress} to determine the effect of
the update.  It only applies if the update counter
is greater than zero, and the \texttt{TConf} component
has a selected next event.

\omitthis{
\begin{small}
\begin{verbatim}  
 crl [evDigress]:
   { tconf di(edig digs, s n)  conf}
   =>
   { tconf1 di(digs edig,n) conf1 }
  if tc(dt, city0, airport, evs,ev, fltil) := tconf
  /\ tconf1 conf1 := applyEvDigress(tconf,conf,edig)
 [print "\nevent digression  " edig "\n ev "  ev] 
 .   
 \end{verbatim}  
 \end{small}
 }
 
 
 A scenario is defined by an initial system configuration \texttt{iSys}, a database of flights
 \texttt{FltDB}, a database of events \texttt{EvDB},
 and an update description.

 A trace \texttt{iSys -TR-> xSys} is a sequence of
 applications of rule instances from the travel rules
 \texttt{TR}, leading from \texttt{iSys} to
 \texttt{xSys}. It is \emph{compliant} if
 \texttt{xSys} satisfies the goal condition
 (\texttt{goal}) that the traveler configuration has
 no remaining events, and no required events have
 been missed. This is formalized by requiring the
 traveler component of \texttt{xSys} to have the form
 \texttt{tc(dt,city,loc,mtE)} since when a required
 event is missed the traveler component is rewritten
 to a term of the form
 \texttt{tcCrit(dt,city,loc,evs,ev,comment)}.
 
 
\longversion{
\input{simple-resilience}
 }
 
\subsection{Checking nab-Resilience}

Checkiing nab-resilience in the travel system is
implemented by the equationally defined function \texttt{isAbRes} using Maude's reflection capability and
strategy language.
\omitthis{
As explained above the execution strategy 
in the rewriting logic travel system advances
time when a flight is
taken or when an event is attended rather that
using a separate rule to advance time one tick (minute)  
at a time.  This means we have a coarse grained notion
of values for ``a'' and ``b''.}
As mentioned above
the upper bound on time is determined by times and durations
of available events and not treated as a parameter to
the algorithm.

The function \texttt{isAbRes} checks n-resilience by first
using \texttt{metaSearch} to find a candidate goal state,
then \texttt{metaSearchPath} gives the corresponding
compliant trace. \footnote{Recall that when execution
reaches a critical state it terminates, so a path to a goal
stat will always be compliant.} The candidate trace is
converted to a rewrite strategy (representing the trace's
list of rule instances). Then the function
\texttt{checkAbRes} iterates through the initial prefixes of
the strategy, using metaSRewrite to follow the trace prefix.
This implements the forall steps in the compliant trace up
to just before the goal. For each state resulting from
executing a prefix, the function \texttt{checkDigs} is
called to apply each one of the available updates (forall
update rules) and then and invoke isAbRes to check for an
n-1 resilient extension trace (exists a suitable trace
extension). If n is zero, \texttt{abResCheck} simply finds a
compliant trace. If the n-1 resilience check fails for some
update after some prefix execution, the current candidate
trace is rejected and \texttt{isAbRes} continues searching
for the next candidate trace. If the continued search for
candidate traces fails then the system under consideration
is not nab-resilient. If the n-1 resilience check succeeds
for every update of every prefix execution, then the
strategy is returned as a witness for nab-resilience.

We tested nab-resilience to flight updates using
instances of the following command.

\begin{small}
\begin{verbatim}  
red isAbRes(['TRAVEL-SCENARIO],N,allDi,SYST,patT,tCond,uStrat,0) .
\end{verbatim}  
\end{small}
\noindent
\texttt{N} is the number of updates (1,2, or 3),
\texttt{SYST} is (the meta representation of) 
an inital state with a starting day that is as late
as possible to succeed if nothing goes wrong (247)
or one day earlier (246) and 2 or 3 events. 
\texttt{patT} and \texttt{tCond} are the metaSearch pattern and condition arguments and \texttt{uStrat} is used
to construct the update rule strategy.
In the summary tables the \texttt{R?} indicates
the result of \texttt{isAbRes}: 
\texttt{Y} for yes (a non-empty strategy is returned)
and \texttt{N} for no.
A dash indicates experiment not done (because
the check fails for smaller N).

\omitthis{iSysT iSysT6 i3SysT i3SysT6}

\begin{small}
\begin{verbatim}  
 N:    1         2        3
2ev    R?  time  R? time  R? time
  247  N   86ms  -        -
  246  Y   81ms  Y  147ms  N 7476ms
3ev 
  247  N 1400ms  -         -
  246  Y  325ms  Y 685ms   NF

Summary of n-ab Resilience to n of 3 flight update rules  
\end{verbatim}  
\end{small}

The experiments for nab-resilience to event updates
are instances of the following command.  The parameters are the same as for flight updates.

\begin{small}
\begin{verbatim}  
red isAbRes(['TRAVEL-SCENARIO],1,allEv,iSysT,patT,tCond,ueStrat,0) .
\end{verbatim}  
\end{small}
\noindent
\texttt{allEv} is the set of all implemented
event update descriptions.

\omitthis{addEv("muc") edEvS(hm(4,0)) edEvD(hm(4,0))}

\begin{small}
\begin{verbatim}  
 N:    1         2        3
2ev    R?  time  R? time  R? time
  247  Y  78ms   N 77ms    -
  246  Y  98ms   N 34800ms -
3ev 
  247  Y 143ms  N 2627ms  -
  246  Y 220ms  Y 633ms   Y 2634ms

Summary of n-ab Resilience to n of 3 event update rules
\end{verbatim}  
\end{small}



==> sections/s4-1-example-short.tex <==
\subsection{Time-bounded resilience: Travel Example}
\label{sec:ex}
To illustrate the concepts introduced in the definitions above, we consider a simplified travel example described in section ~\ref{sec:motivation}. 

\begin{remark}
\label{remark: example-pts}
It is easy to check that this example planning scenario described below is progressing. Note that, taking into account Remark \ref{remark: pts}, we do not write the empty facts nor the sets of time constraints~$\Cscr_r$. 
\end{remark}

\paragraph{Initial configuration.}
The initial configuration contains the facts specifying the multiple flight combinations from San Francisco to Dubrovnik available, via the given set of direct flights between the cities of San Francisco, Frankfurt, Zagreb and Dubrovnik.
For example, the fact $\Flight(15,\SanFran, FRA, \LH, 455, 21:40,650)@0 $ denotes the Lufthansa direct flight 455 from San Francisco to Frankfurt, labeled with the identifier 16, which departs at 21:40 with a flight duration of 650 minutes. Similarly, the fact $\FlightAv(2,\SanFran, \DBV, 16,14,0)@0$ specifies the connection of 2 flights: Flight with identifier 16, followed by flight with identifier 14.
%In addition, the initial configuration denotes that there are several events to attend. The facts $\Event(\main,215, 12:00, 1)@0, \Done(\no, 1)@0$ specifies the main event or a task that is scheduled at noon of the 215th day and has not yet been performed, \eg, the researcher has yet to present his work at the conference.

\vspace{5pt}
\noindent
\paragraph{System rules}
\begin{scriptsize}
\[
\begin{array}{l}

 \hspace{-1em} r_2: \textbf{Select 2-flights connection:}\\[3pt]
\Time@T, \City_0(c_0)@T_0, \City_1(c_1)@T_1, \SegMax(n+1)@T_2,
\FlightAv(2, x_1,x_2,0)@T_3,  \Leq,(2,n+1)@T_4,\\
\qquad
\Flight(x_1,c_0,y,h_1:m_1,d_1)@T_5, \Flight(x_2,y,c_1,h_2:m_2,d_2)@T6,

 \Selected(\no)@T_8
%\, \mid \, %oMove\,(Id,X,Y,E+1,T,T_1,\ldots,T_n,north)  
\\
\qquad \qquad \lra \Time@T, 
\City_0(c_0)@T_0, \City_1(c_1)@T_1, \SegMax(n+1)@T_2,
\FlightAv(2, x_1,x_2,0)@T_3,  \\
\qquad  \qquad \qquad \
\Leq,(2,n+1)@T_4,
\Flight(x_1,c_0,y,h_1:m_1,d_1)@T_5, \Flight(x_2,y,c_1,h_2:m_2,d_2)@T6,
 \\
\qquad \qquad \qquad \
\Selected(\ok)@(T+1), \Con(x_1)@T, \Con(x_2)@T\\[5pt]
 
\hspace{-1em} r_4: 
\textbf{Get to the airport:}\\[3pt]
\Time@T, \City_0(x)@T_0, \Selected(\ok)@T_1, \At(x, \Center)@T_2 \, \mid \, T_2 \leq T  \\
\qquad \qquad \lra 
\Time@T, \City_0(x)@T_0, \Selected(\ok)@T, \At(x, \airport)@(T+D_{\shuttle})
 \\[5pt]
 \hspace{-1em} r_5: 
 \textbf{Take the flight:} \ \ %\emph{ - allow at least 30 mins for boarding}
 \\[3pt]
\Time@T,  \Clock(h:m)@T_1, \At(x, \airport)@T_2, 
\Flight(a,x,y,h:m,d)@T_3,  \Con(a)@T_4
\, \mid \, T_2+30 \leq  T  %oMove\,(Id,X,Y,E+1,T,T_1,\ldots,T_n,north)  
\\
\qquad \qquad \lra 
\Time@T, \Clock(h:m)@T_1,  \At(y, \airport)@(T+d),  \Flight(a,x,y,h:m,d+30)@T_3
  \\[5pt]
\hspace{-1em} r_7: 
 \textbf{Attending events:}\\[3pt]
\Time@T, \Clock(h:m)@T_1, \Day(y)@T_2, \At(x, \Center)@T_3, City_1(x)@T_4, 
\\ \qquad
\Event(a,y,h:m,i)@T_5, \Done(\no,i)@T_6
%\, \mid \, T_2 \leq T 
\\ 
\qquad \qquad \lra 
\Time@T, \Clock(h:m)@T_1, \Day(y)@T_2,  \At(x, \Center)@T_3,  City_1(x)@T_4,
\\ \qquad \qquad \qquad\
\Event(a,y,h:m,i)@(T+1),  \Done(\yes,i)@T
 %\\[5pt]
\end{array} 
\] 
\end{scriptsize}

Using a rule $r_2$, the researcher selects the available connecting flights. The preference of at most 2 flights is specified using the fact $\SegMax(n)$ denoting the maximum number of connecting flights $n$.
%The application of such a rule also indicates that the flight selection has been made by replacing the fact $\Selected(\no)@(T+1)$ with the fact $\Selected(\ok)@(T+1)$.
%
Rule $r_4$ specifies that the traveler needs one $D_{shuttle}$ minutes to get from the departing city center to the airport, while rule $r_5$
specifies that once at the airport, the traveler needs at least 30 minutes to board a plane (specified by the time constraint $T_2 +30\leq T$), take the flight for its duration to arrive at the destination.
Once at the next airport, the traveler needs at least 30 minutes to board the next flight.
When the airport of the final destination is reached, it takes at least another 30 minutes to take the connecting ride to the city center, and then another $D_{shuttle}$ minutes for the transfer itself, as specified by the rule $r_6$.
%
The rule $r_7$ specifies that a researcher participates in the planned activities if he is on site at the time of the event.

\noindent
\paragraph{System time maintenance rules}
\begin{scriptsize}
\[
\begin{array}{l}
\hspace{-1em}  \textbf{Advance clock:}\\[3pt]
t_1: 
\Time@T, Clock(h:m)@T_1, \Leq(m,58)@T_2 \, \mid \, T_1 = T
%\, \mid \, T_1 \leq T  %oMove\,(Id,X,Y,E+1,T,T_1,\ldots,T_n,north)  
%\\ \qquad \qquad 
\lra
\\ \qquad \quad
\Time@T, \Clock(h:m+1)@(T+1), \Leq(m,58)@T_2
\\[3pt] t_2: 
\Time@T, \Clock(h:59)@T_1, \Leq(h,22)@T_2 \, \mid \, T_1 = T
%\, \mid \, T_1 \leq T  %oMove\,(Id,X,Y,E+1,T,T_1,\ldots,T_n,north)  
%\\ \qquad \qquad 
\lra 
\\ \qquad \quad
\Time@T, \Clock(h+1:00)@(T+1), \Leq(h,22)@T_2
\\[3pt] t_3: 
\Time@T, \Clock(23:59)@T_1, \Day(x)@T_2 \, \mid \, T_1 =T
%\, \mid \, T_1 \leq T  %oMove\,(Id,X,Y,E+1,T,T_1,\ldots,T_n,north)  
%\\ \qquad \qquad 
\lra
\\ \qquad \quad
\Time@T, \Clock(00:00)@(T+1), \Day(x+1)@T
\end{array} 
\] 

\end{scriptsize}

The rules $t_1, t_2$ and $t_3$ ensure that $\Clock$ is synchronized with the global time.
The rules $t_1, t_2$, and $t_3$ set the time value displayed by the $\Clock$ so that it synchronizes with the global time as time progresses.
For technical reasons related to the form of the PTS rules (rules create at least one fact with the timestamp greater than the global time), the timestamp of the fact $\Clock$ is one time unit greater than the global time. This does not affect the modeling of time features in the formalism, such as the time of events, the duration of actions, etc.

\noindent
\paragraph{Update rules}

Due to some external causes beyond the control of the traveler, some unpredictable events may lead to interruptions in the itinerary. For simplicity, we model only one type of update rule, namely flight delays. More specifically, an application of an update rule models a flight being delayed by 30 minutes.

%, without entering into reasons for flight delays.


\begin{scriptsize}
\[
\begin{array}{l}
\hspace{-1em}\textbf{Flight being delayed for 30 mins:}\\[3pt]
\Time@T, \Flight(a,x,y,h:m,d)@T_1
%\, \mid \, T_1 \leq T  %oMove\,(Id,X,Y,E+1,T,T_1,\ldots,T_n,north)  
%\\ \qquad \qquad 
\lra Time@T,   \Flight(a,x,y,(h:m) + (0:30),d)@(T+1)
\end{array} 
\] 

\end{scriptsize}

In the above rule, we assume that the operation $+$ is naturally defined for values representing time in hours and minutes. 




\vspace{5pt}
\noindent
\paragraph{Critical configuration specification:}

%\vspace{5pt}
%{\small 
%- forcing that $\Clock$ has timestamp as $\Time$ plus 1 (+1 to have PTS Advance clock rules):}
\begin{scriptsize}
\[
\begin{array}{l}
\hspace{-1em}\textbf{Missing the main event}:\\[2pt]
\langle \{ %\Time@T,
\Clock(h:m)@T_1, \Day(x)@T_2, 
\Event(\main,x,h_1:m_1,i)@T_3,  \Done(\no,i)@T_4, 
\\ \qquad \ \Leq(h_1:m_1, h:m)@T_5\} , \emptyset\rangle
\\[8pt]
\hspace{-1em}\textbf{Missing two auxiliary events}:\\[2pt]
\langle \{ %\Time@T,
\Clock(h:m)@T_1, \Day(x)@T_2, 
\Event(\aux,x,h_1:m_1,i)@T_3, \Event(\aux,x,h_2:m_2,j)@T_4, \\ \quad \
\Done(\no,i)@T_5,  \Done(\no,j)@T_6,
\Leq(h_1:m_1, h:m)@T_5, \Leq(h_2:m_2, h:m)@T_6 \} , \emptyset\rangle
\\ \qquad \
\qquad - \text{events on the same day}
\\[8pt]
\langle \{ %\Time@T,
\Clock(h:m)@T_1, \Day(x)@T_2, 
\Event(\aux,x_1,h_1:m_1,i)@T_3, \Event(\aux,x,h_2:m_2,j)@T_4,
\\ \quad \
\Done(\no,i)@T_5,  \Done(\no,j)@T_6,
 \Leq(h_2:m_2, h:m)@T_5, \Leq(x_1+1,x)@T_6\} , \emptyset\rangle  \qquad \ \
 \\ \qquad \
 \qquad - \text{events not on the same day}
\\[8pt]
\hspace{-1em}\textbf{Event Admin / Maintenance:}\\[3pt]
\langle \{ \Time@T, \Clock(h:m)@T_1, \Day(x)@T_2, \At(y,\Center), \City_1(y),
\\ \qquad \
\Event(a,x,h:m,i)@T_3, \Done(\no,i)@T_4
, \{ T_1 = T\} \rangle
\\[2pt]
\qquad  \text{- forcing that  an $\Event$ is attended when on the location at the time of the event (normally $T_1 = T+1$)}
\\[8pt]
\hspace{-1em}\textbf{Clock Admin / Maintenance:}\ \ %[3pt]
\langle \{ \Time@T, Clock(h:m)@T_1\} , \{ T_1 < T\} \rangle
\\[2pt]
\qquad  \text{- forcing that $\Clock$ has timestamp as $\Time$ plus 1 (+1 to have PTS Advance clock rules)}

\end{array} 
\] 

\end{scriptsize}

\vspace{1em}
It is critical not to participate in the main event. It is also critical to miss two side activities.
Due to the nature of the MSR formalism, we use a critical configuration specification to enforce the application of rules, and then consider non-critical traces.
By $\Clock$ maintenance critical configuration specification, we ensure that $\Clock$ is synchronized with the global time in the non-critical traces. In that way we enforce the application of rules $t_1, t_2$, and $t_3$ that increase the time value displayed by the $\Clock$, to match the global time.

It is similarly critical if a researcher is on site at the time of planned activity and does not participate. In this way, we force participation in events when the researcher is present. For a more detailed specification, we could similarly model the researcher's conscious decisions not to participate in some side activities and not count them as missed activities in this case.

\vspace{3pt}
\noindent
\paragraph{Goal:}
\vspace{1em}
In this example, the goal is for the researcher to attend the main event, which is the main purpose of the trip.



%\vspace{5pt}
%{\small 
%- forcing that $\Clock$ has timestamp as $\Time$ plus 1 (+1 to have PTS Advance clock rules):}
\begin{scriptsize}
\[
\begin{array}{l}
\hspace{-1em}\textbf{Getting to the main event}:\ \ %[2pt]
\langle \{ %\Time@T,
\Clock(h:m)@T_1, \Day(x)@T_2, 
\Event(\main,x,h_1:m_1,yes)@T_3\} , \emptyset\rangle
\\[5pt]

\end{array} 
\] 

\end{scriptsize}


For reasons of readability and to simplify the presentation, in the above formalization, we have only listed a few cities (San Francisco, Frankfurt, Zagreb, Dubrovnik) and the connecting flights in the example. We also assume a fixed daily flight schedule. %  ... specifications contain exactly one
Generalizing to a broader flight database and a more detailed travel process (modeling baggage handling, customs control, etc.) is straightforward, by including specific predicates and rules. Since we primarily want to demonstrate resilience properties, we abstract away from such details and focus on the parameters and the notions included in our definitions of resilience properties.
